Complexity and Applications of Edge-Induced Vertex-Cuts

Motivated by hypergraph decomposition algorithms, we introduce the notion of edge-induced vertex-cuts and compare it with the well-known notions of edge-cuts and vertex-cuts. We investigate the complexity of computing minimum edge-induced vertex-cuts and demonstrate the usefulness of our notion by applications in network reliability and constraint satisfaction.

==> graphics/ex_genhgraph.tex <==

\begin{figure}[t]
\begin{center}
 
\input{graphics/ex_genhgraph.pstex_t}
\hspace*{0.8cm}
\input{graphics/ex_hyptree.pstex_t}

\caption{Example of a hypergraph and its generalized hypertree decomposition}
\label{fig:ex_genhgraph}
\end{center}
\end{figure}



==> graphics/ex_gmincuts.tex <==

%\begin{figure}[t]
\begin{center}
 
\input{graphics/ex_gmincuts.pstex_t}

\caption{Graph example}
\label{fig:ex_gmincuts}
\end{center}
%\end{figure}



==> graphics/ex_intro.tex <==

\begin{figure}[t]
\begin{center}
 
\input{graphics/ex_intro.pstex_t}

\caption{Graph example to illustrate mincuts}
\label{fig:ex_intro}
\end{center}
\end{figure}



==> graphics/ex_mincuts.tex <==

%\begin{figure}[t]
\begin{center}
 
\input{graphics/ex_mincuts.pstex_t}

\caption{Hypergraph example}
\label{fig:ex_mincuts}
\end{center}
%\end{figure}



==> graphics/proof.tex <==

\begin{figure}[t]
\begin{center}
 
\input{graphics/proof.pstex_t}

\caption{Encoding of the 3SAT instance $\{\{x, \neg y, z\}, \{x, \neg y, \neg z\}\}$}
\label{fig:proof}
\end{center}
\end{figure}


